Unified approach for computing sum of sources over CQ-MAC

We consider the task of communicating a generic bivariate function of two classical sources over a Classical-Quantum Multiple Access Channel (CQ-MAC). The two sources are observed at the encoders of the CQ-MAC, and the decoder aims at reconstructing a bivariate function from the received quantum state. Inspired by the techniques developed for the analogous classical setting, and employing the technique of simultaneous (joint) decoding developed for the classical-quantum setting, we propose and analyze a coding scheme based on a fusion of algebraic structured and unstructured codes. This coding scheme allows exploiting both the symmetric structure common amongst the sources and the asymmetries. We derive a new set of sufficient conditions that strictly enlarges the largest known set of sources (capable of communicating the bivariate function) for any given CQ-MAC. We provide these conditions in terms of single-letter quantum information-theoretic quantities.

==> MATH_template.tex <==
%\documentclass[9pt]{article}
%\usepackage[utf8]{inputenc}
%\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{tikz}
%\usepackage{mathdots}
\usepackage[utf8]{inputenc}
%\usepackage[ margin=1in ]{geometry}
\usepackage{amsfonts} 
\usepackage{epstopdf}
%\usepackage{mathtools}
\usepackage{graphicx}
%\usepackage{relsize}
%\usepackage{xy}
%\input{xypic}
\usepackage{bbm}
%\setlength{\footskip}{20pt}
\usepackage{enumerate}
\usepackage{epsf,epsfig,verbatim,amssymb,amsmath,array,cite,amsthm,subfigure,multicol,multirow}  
\usepackage{psfrag,bm,xspace}
%\usepackage{slashbox}
\usepackage{hhline}
\usepackage{mathabx}
\usepackage{physics}
%\evensidemargin=-0.2in \oddsidemargin=-0.2in \topmargin=-0.1in \textwidth=6.7in \textheight=9in \columnsep=0.30in
%\parindent 0.5cm
%\baselineskip=1.0\normalbaselineskip
%\renewcommand{\baselinestretch}{1.27}
\pagestyle{plain}



\newcommand{\prodin}{\prod_{i=1}^n}
\newcommand{\sumin}{\sum_{i=1}^n}
\newcommand{\ra}{\rightarrow}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\mc}{\mathcal}
\newcommand{\mb}{\mathbb}
\newcommand{\bs}{\boldsymbol}
\newcommand{\e}{\epsilon}
\newcommand{\dl}{\delta}
\newcommand{\g}{\gamma}
\newcommand{\rtq}{\tilde{R}_{\mathcal{Q}}}

\newtheorem{thm}{Theorem}
\newtheorem{dfn}{Definition}
\newtheorem{rem}{Remark}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{fact}{Fact}



\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
%\newtheorem{lem}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{definition}{Definition}

\theoremstyle{definition}
\newtheorem{example}{Example}
\newtheorem{conjecture}{Conjecture}
\newtheorem{question}{Question}
\newtheorem{problem}{Problem}
\newtheorem*{prob*}{Problem}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{rems}{Remarks}
\newtheorem{para}{}
\newtheorem{summary}{Summary}



%-----------------------------------------------------------------------------------------

%\addtolength{\hoffset}{-3cm} \addtolength{\textwidth}{5.5cm}
%\addtolength{\voffset}{-1.0cm} \addtolength{\textheight}{4cm}

\allowdisplaybreaks % makes automatic splits of equations

%\theoremstyle{plain}




\renewcommand{\Re}[1]{\ensuremath{\operatorname{Re}\left\{#1\right\}}}
\renewcommand{\Im}[1]{\ensuremath{\operatorname{Im}\left\{#1\right\}}}

\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}

\global\long\def\Z{\mathrm{{\bf Z}}}
\global\long\def\N{\mathrm{{\bf N}}}
\global\long\def\Gal{\mathrm{Gal}}





\global\long\def\RR{\mathbb{R}}
\global\long\def\CC{\mathbb{C}}
\global\long\def\NN{\mathbb{N}}
\global\long\def\QQ{\mathbb{Q}}
\global\long\def\ZZ{\mathbb{Z}}
\global\long\def\EE{\mathbb{E}}
\global\long\def\PP{\mathbb{P}}
\global\long\def\FF{\mathbb{F}}
\global\long\def\11{\mathbbm{1}}
\global\long\def\normal{\triangleleft}
\global\long\def\+{\oplus}

\global\long\def\P{\mathsf{P}}

 \global\long\def\dd{\cdots}
\global\long\def\normal{\triangleleft}
\global\long\def\deq{\delequal}
\global\long\def\tensor{\otimes}
\global\long\def\bigtensor{\bigotimes}

\newcommand*{\Scale}[2][4]{\scalebox{#1}{\ensuremath{#2}}}%


\allowdisplaybreaks% makes automatic splits of equations





%\begin{document}
%
%\title{Information rates of densely sampled Gaussian data: Distributed
%  vector quantization and scalar quantization with transforms.
%\footnote{This work was supported by NSF grant CCF-0329715 and CCF-0448115. 
%This work was presented in part at the IEEE
%  International Conference on Acoustics Speech and Signal Processing
%  (ICASSP), Toulouse, France, May 2006,  and IEEE International Symposium on
%  Information Theory (ISIT), Nice, France,  June/July 2007.
%}}
%\author{David L. Neuhoff  and S. Sandeep Pradhan \\
%Dept. of Electrical Engineering and Computer Science \\
% Univ. of  Michigan, Ann Arbor, MI. \\ December 6, 2010. \\}
%\date{}
%
%\maketitle \thispagestyle{empty} \pagestyle{plain}
%

